Experimental Tests of Particle Flow Calorimetry

Precision physics at future colliders requires highly granular calorimeters to support the Particle Flow Approach for event reconstruction. This article presents a review of about 10 - 15 years of R\&D, mainly conducted within the CALICE collaboration, for this novel type of detector. The performance of large scale prototypes in beam tests validate the technical concept of particle flow calorimeters. The comparison of test beam data with simulation, of e.g.\ hadronic showers, supports full detector studies and gives deeper insight into the structure of hadronic cascades than was possible previously.

==> Realproto.tex <==
\section{Realistic prototypes%
% Put \label in argument of \section for cross-referencing
\label{sec:Realproto}}

{\it Felix, Andy, Roman, Jos\'e 5p}

\begin{itemize}
\item 
Introduction: challenges
\item
SiD ECAL {\it Andy 1p}
\item
ILD ECAL and ROC ASICs {\it Roman 1p}
\item
Scintillator ECAL and AHCAL {\it Felix 1p}
\item
Gasous HCAL {\it Andy, Roman, Jos\'e 1p}
\end{itemize}


